Treeffuser: Probabilistic Predictions via Conditional Diffusions with Gradient-Boosted Trees

Probabilistic prediction aims to compute predictive distributions rather than single point predictions. These distributions enable practitioners to quantify uncertainty, compute risk, and detect outliers. However, most probabilistic methods assume parametric responses, such as Gaussian or Poisson distributions. When these assumptions fail, such models lead to bad predictions and poorly calibrated uncertainty. In this paper, we propose Treeffuser, an easy-to-use method for probabilistic prediction on tabular data. The idea is to learn a conditional diffusion model where the score function is estimated using gradient-boosted trees. The conditional diffusion model makes Treeffuser flexible and non-parametric, while the gradient-boosted trees make it robust and easy to train on CPUs. Treeffuser learns well-calibrated predictive distributions and can handle a wide range of regression tasks -- including those with multivariate, multimodal, and skewed responses. We study Treeffuser on synthetic and real data and show that it outperforms existing methods, providing better calibrated probabilistic predictions. We further demonstrate its versatility with an application to inventory allocation under uncertainty using sales data from Walmart. We implement Treeffuser in https://github.com/blei-lab/treeffuser.

==> sections/2-review-old.tex <==
\glsreset{gbt}
\glsreset{sde}
\section{Background}
\label{sec:background}
Treeffuser combines two ideas: diffusion models and \glspl{gbt}. This section provides a gentle introduction to both topics. Familiar readers can skip ahead to \Cref{sec:treeffuser}.

% If you know both, you can go to . We begin by reviewing how diffusion models can be used to learn the marginal distribution $\pi$ of a random variable $\bs{y} \in \R^{d_y}$. Next, we discuss how gradient-boosted trees can model a scalar random variable $a$ as a function of another one $\bs{b} \in \R^{d_b} $. 

% A diffusion model is a generative model that consists of two processes, a forward diffusion, and a reverse diffusion. The forward process takes an unknown distribution target $\pi(\bs{y})$ and continuously transforms it into a simple distribution $p_\text{simple}(\bs{y})$, typically a Gaussian. It does so by progressively adding noise to samples from $\pi$, such as our data. 
% The reverse process transforms the simple distribution into the target distribution, effectively denoising any perturbed samples from $\psimple$. One way to learn this noising-denoising process is to estimate the \textit{score function}, the gradient of the log probability of the noisy data with respect to the data itself. Once the diffusion model is learned, we can access the target distribution $\pi$: first draw samples from $p_\text{simple}$ and then use the reverse transformation, as guided by the score, to map them back to $\pi$.
\subsection{Diffusion Models}
\label{sec:bac-diffusions}
% not sure about this sentence
% Given an unknown target distribution $\pi(\bs{y})$, a diffusion model is a generative process that aims to model $\pi(\bs{y})$.
A diffusion model is a generative model that consists of two processes, a forward diffusion, and a reverse diffusion. The forward process takes an unknown distribution target $\pi(\bs{y})$ and continuously transforms it into a simple distribution $p_\text{simple}(\bs{y})$, typically a Gaussian. It does so by progressively adding noise to samples from $\pi$, such as our data. 

The reverse process transforms the simple distribution back into the target distribution by denoising any perturbed samples from $\psimple$. 
If it is possible to learn the reverse process, then we can effectively access the target distribution $\pi$: first draw samples from $p_\text{simple}$ and then use the reverse transformation, as guided by the score, to map them back to $\pi$.

One way to learn this noising-denoising process is to estimate the \textit{score function}, the gradient of the log probability of the noisy data with respect to the data itself.

We detail the three main components of score-based diffusions--the forward process, the reverse process, and the estimation of the score function--below.

\parhead{The forward diffusion process.}
A diffusion model is described by the following generative process:
\begin{equation}
    \left\{ \begin{array}{l}
        \text{Draw } \bs{y}(0) \sim \pi, \\
        \text{Evolve $\bs{y}(t)$ until $T$ according to: } ~\text{d} \bs{y}(t) = f(\bs{y}(t), t) \text{d}t + g(t) \text{d}\bs{w}(t),
    \end{array} 
    \right. \label{eq:sde_forward}
\end{equation}
% \begin{enumerate}[leftmargin=0.5cm]
%     \item Draw $\bs{y}(0) \sim \pi$
%     \item Evolve $\bs{y}(t)$ according to a stochastic differential equation (SDE) until $t = T$ 
%     \begin{align}
%         \text{d} \bs{y}(t) = f(\bs{y}(t), t) \text{d}t + g(t) \text{d}\bs{w}(t), \label{eq:sde_forward}
%     \end{align} 
where the process of evolving the \gls{sde} involves a standard Brownian motion $\bs{w}(t)$ and model parameters $f: \mathbb{R}^{d_y} \times [0, T] \to \mathbb{R}^{d_y}$ 
    and $g: [0, T] \to \mathbb{R}$, respectively called the \textit{drift} and \textit{diffusion} functions.
% \end{enumerate}

The SDE in \cref{eq:sde_forward} determines the evolution of $\bs{y}(t)$ over time, thereby inducing a distribution of $\bs{y}(t)$ at each $t$, that we write $p_t(\bs{y}(t))$. We further write the distribution of $\bs{y}(t)$ conditional on another $\bs{y}(u)$ as $p_{ut}(\bs{y}(t) \mid \bs{y}(u))$.
In practice, $f$ and $g$ are simple functions such that  $p_{0t}(\bs{y}(t) \mid \bs{y}(0))$ has a closed form. In fact, if the drift $f$ is affine in $\bs{y}(t)$ and the diffusion function $g$ is a scalar that does not depend on $\bs{y}(t)$, the distribution $p_{0t}$ is always Gaussian, with a mean we write $m(t;\bs{y}(0))$ and a covariance multiple of the identity we write $\sigma(t)^2 I$.

The time horizon $T$ is chosen such that the resulting marginal distribution $p_T(\bs{y}(T)) = \int_{\bs{y'}} p_T(\bs{y}(T) \mid \bs{y}(0)=\bs{y}')\pi(\bs{y}') \text{d}\bs{y}'$ is a simple distribution $p_\text{simple}$ agnostic to what $\pi$ was. The intuition is that as the diffusion progresses, the initial density $\pi$ is forgotten.

We detail our choice of $f$, $g$ and $T$ in Appendix \cref{apx:sec:data-driven-hyperparameters}, this choice corresponds to the variance exploding SDE (VESDE) in \citet{song2020score}, and induces a trivial closed form expression for the functions $m$ and $\sigma$.



There are no model parameters to learn in the diffusion model, and the conditional distributions
$p_{0t}(\bs{y}(t) \mid \bs{y}(0))$ are trivial to compute. The challenge is to learn how to compute (or sample from) the
conditional distribution $p_{Tt}(\bs{y}(t) \mid \bs{y}(T))$. This is called \textit{reversing} the diffusion process. Knowing $p_{Tt}$ is key to learning the
target distribution $\pi$ because it can be written as $\pi(\bs{y}(0)) = \mathbb{E}_{p_T}[p_{T0}(\bs{y}(0) \mid \bs{y}(T))]$ where $p_{T} = p_\text{simple}$ is known.

\parhead{The reverse diffusion process.} 
Consider the following SDE that is reversed in time from $T$ to $0$,
\begin{equation}
    \left\{ \begin{array}{l}
\tilde{\bs{y}}(T) \sim p_\text{simple}, \\
\text{d} \tilde{\bs{y}}_t = [f(\tilde{\bs{y}}(t), t) - g(t)^2 \nabla_{\tilde{\bs{y}}(t)} \log p_t(\tilde{\bs{y}}(t))] \text{d}t + g(t) \text{d}\tilde{\bs{w}}(t),         
    \end{array}
    \right. \label{eq:sde_reverse}
\end{equation}
where $\tilde{\bs{w}}(t)$ is a standard Brownian with reversed time and $p_t$ is the density of $\bs{y}(t)$ defined by the forward \gls{sde} (\ref{eq:sde_forward}). Similar to the forward case, the reverse \gls{sde} induces a distribution $\tilde{p}_t$ for $\tilde{\bs{y}}(t)$ at each $t$. \citet{anderson1982reversediffusions} shows that, if we denote by $\tilde{p}_{Tt}$ the conditional distribution of $\tilde{\bs{y}}(t)$ given $\tilde{\bs{y}}(T)$, then $\tilde{p}_{Tt} = p_{Tt}$ for any time $t$. In other words, $\tilde{\bs{y}}(t) \mid \tilde{\bs{y}}(T) = \bs{a}$ and $\bs{y}(t) \mid \bs{y}(T) = \bs{a}$ have the same distribution for all $\bs{a}$. Since we designed the diffusion such that $p_T \approx p_\text{simple} = \tilde{p}_T$, we have in particular $\tilde{\bs{y}}(t) \sim \bs{y}(t)$.

\Gls{sde} solvers let us sample from distributions that are solutions of \gls{sde}; hence, we can obtain samples of $\pi(\bs{y})$ by solving \cref{eq:sde_reverse}.
However, the function $\bs{y} \mapsto \nabla_{\bs{y}} \log p_t(\bs{y})$, called the \textit{score}, is usually unknown and needs to be estimated.

\parhead{Estimating the score.} \citet{Vincent2010} shows that the score can be estimated from trajectories of the \gls{sde} as the minimizer of the following objective function:  
\begin{align}
    [\bs{y} \mapsto \nabla_{\bs{y}} \log p_t(\bs{y})] = \argmin_{s \in \mathcal{S}}  \EE_{t}\EE_{\pi}\EE_{p_{0t}} \left[ \left\| \nabla_{\bs{y}(t)} \log p_{0t}(\bs{y}(t)\mid \bs{y}(0)) - s(\bs{y}(t), t) \right\|^2 \right] \label{eq:estimate-score},
\end{align}
where $\mathcal{S} = \{ s: \mathbb{R}^{d_y} \times [0, T] \to \mathbb{R}^{d_y} \}$ is the set of all possible score functions
indexed by time $t$, and $\EE_{t}$ can be an expectation over any distribution of $t$ whose support is exactly $[0, T]$. 
Since $p_{0t}$ is a normal distribution $\mathcal{N}(m(t; \bs{y}(0)), \sigma(t)^2 I)$, we have
\begin{align}
    \nabla_{\bs{y}(t)} \log p_{0t}(\bs{y}(t) \mid \bs{y}(0)) = \frac{m(t; \bs{y}(0)) - \bs{y}(t)}{\sigma(t)^2}. \label{eq:score-trivial}
\end{align}

In practice, the expectations in \cref{eq:estimate-score} are approximated using the empirical distribution formed by the observed $\bs{y}$ for $\mathbb{E}_{\pi}$, and by sampling the simple and known forward \gls{sde} trajectories $\bs{y}(t) \mid \bs{y}(0)=\bs{y}$ for $\mathbb{E}_{p_{0t}}$.
The objective can then be minimized by parametrizing $s$ with any function approximator, e.g., a neural network.
The obtained score estimator can then be used to reverse the diffusion process and estimate the target distribution $\pi(\bs{y})$.


\subsection{Gradient Boosted Trees} 
Consider the following common machine learning task. Given variables $(\bs{a}, b) \sim \pi$, where $b$ is scalar, our goal is to learn the function $F^*(\bs{a})$ that best approximates $b$ from $\bs{a}$:
\begin{equation}
    F^* = \argmin_{F} \EE_{(\bs{a}, b)\sim \pi}\left[L(F(\bs{a}), {b})\right], \label{eq:boosting_global_objective}
\end{equation} 
where $L$ is a loss function measuring the quality of $F$, e.g., the square loss $L(u,v) = (u-v)^2$.
\glsreset{gbt}
\Glspl{gbt} are a widely used non-parametric machine learning model for this task  \citep{friedman2001greedy}. \Glspl{gbt} use decision trees \citep{hastie2009elements} as simple building block functions $f: \mathbb{R}^d \to \mathbb{R}$ to form a good approximation $\hat{F}$ of $F^*$. 
\Glspl{gbt} sequentially build approximations $\hat F_i$ defined as 
\begin{align}%\textstyle
    \hat{F}_i(\bs{a}) = \sum_{m = 0}^{i-1} \varepsilon f_m(\bs{a}),
\end{align} with increasingly more decision trees and where $\varepsilon \in (0,1)$ is a parameter akin to a learning rate.

Each decision tree $f_i$ is constructed to minimize the squared error between the current approximation $\hat{F}_i$ and the gradient of the loss function:
\begin{align}
    f_i = \argmin_{f \in \texttt{Trees}} \EE_{\bs{a}, b} \left[\Bigl( f(\bs{a}) + \frac{\partial L(F_i(\bs{a}),b)}{\partial F_i(\bs{a})} \Bigr)^2\right]. \label{eq:boosting_local_eq}
\end{align}

As the number of trees $i$ increases, the approximation $\hat{F}_i$ becomes a better minimizer of \cref{eq:boosting_global_objective}. The training is usually stopped when the loss function no longer improves on a validation set.

Various modifications to this basic algorithm have been proposed, including several methods based on different loss functions in \cref{eq:boosting_global_objective}, higher order optimizations for \cref{eq:boosting_local_eq} and general heuristics for faster training \citep{chen2016xgboost, ke2018lightgbm, prokhorenkova2019catboost}. 


==> sections/7-ack.tex <==
\section*{Acknowledgements}
N.B. and D.B. were funded by NSF IIS-2127869, NSF DMS-2311108, NSF/DoD PHY-2229929, ONR N00014-17-1-2131, ONR N00014-15-1-2209, the Simons Foundation, and Open Philanthropy.
A.N. was supported by funding from the Eric and Wendy Schmidt Center at the Broad Institute of MIT and Harvard, and the Africk Family Fund.
A.A.G. was supported by The Halvorsen Center for Computational Oncology at the Memorial Sloan Kettering Cancer Center.
The authors thank Brian Trippe for insightful discussions and Luhuan Wu for helpful comments on the manuscript.
The authors also thank Calvin McCarter for valuable feedback on the usability of the Python package.
